Controlling Text Complexity in Neural Machine Translation

This work introduces a machine translation task where the output is aimed at audiences of different levels of target language proficiency. We collect a high quality dataset of news articles available in English and Spanish, written for diverse grade levels and propose a method to align segments across comparable bilingual articles. The resulting dataset makes it possible to train multi-task sequence-to-sequence models that translate Spanish into English targeted at an easier reading grade level than the original Spanish. We show that these multi-task models outperform pipeline approaches that translate and simplify text independently.

==> backup.tex <==
\subsection{Monolingual Text Simplification}

\mc{Reviewer: ``Where does this come from? Is this the second part of the pipeline? Why not evaluate the first part as well?'' I wonder whether this should be moved to Supplemental material.}

We first establish that our model configuration is sound by comparing our model with prior work on  Monolingual Text Simplification. As can be seen in table~\ref{tab:resultsmono}, our implementation yields BLEU and SARI score that are close to those reported in \newcite{ScartonSpecia2018}. The difference in Flesch score can be attributed to changes in the number and complexity of articles available in Newsela at the time the datasets were extracted. Our version of corpus has 460k pairs compared to 550k instance pairs used by \cite{ScartonSpecia2018} because of changes to the content of Newsela. Higher value of Flesch score implies better readability of the text. Table \ref{missing} shows the grade distribution of missing articles from our version of Newsela. Many articles that are not available in our corpus belong to lower grade levels, thus lowering the Flesch score for our model. Using Byte-pair Encoding (BPE) to segment words into subword units \cite{SennrichHaddowBirch2016a} further boosts the SARI score by a large margin. 

\begin{table*}[ht]
\centering
\begin{tabular}{|l|l|l|l|}
 \hline
Model & Bleu & SARI & Flesch \\
    \hline
\multicolumn{4}{|l|}{Results copied from \newcite{ScartonSpecia2018}}\\
  seq2seq w/ side-constraint  & 62.91 & 41.01 & 82.91  \\
  \hline
\multicolumn{4}{|l|}{Reimplementation evaluated on our Newsela download}\\ 
seq2seq w/ side-constraint & 58.61 & 39.81  & 70.44\\
seq2seq w/ side-constraint + BPE  & 61.87	& 52.78 & 66.98\\
\hline
\end{tabular}
\caption{Comparison with previously published results on Newsela English text simplification
%\mc{Is the test set exactly the same in all of these comparisons or not?}
}\label{tab:resultsmono}
\end{table*}

==> images/xling-write.tex <==
% comments
\usepackage{xcolor}
\newcommand{\ensuretext}[1]{#1}
%Marine
\newcommand{\mcmarker}{\ensuretext{\textcolor{magenta}{\ensuremath{^{\textsc{M}}_{\textsc{C}}}}}}
%Xing
\newcommand{\xnmarker}{\ensuretext{\textcolor{blue}{\ensuremath{^{\textsc{X}}_{\textsc{N}}}}}}
%Marianna
\newcommand{\mjmarker}{\ensuretext{\textcolor{cyan}{\ensuremath{^{\textsc{M}}_{\textsc{M}}}}}}
%Kevin
\newcommand{\kdmarker}{\ensuretext{\textcolor{purple}{\ensuremath{^{\textsc{K}}_{\textsc{D}}}}}}
%Paul
\newcommand{\jpmmarker}{\ensuretext{\textcolor{green}{\ensuremath{^{\textsc{P}}_{\textsc{M}}}}}}
%Sweta
\newcommand{\samarker}{\ensuretext{\textcolor{orange}{\ensuremath{^{\textsc{S}}_{\textsc{A}}}}}}
%enable comments here
%\newcommand{\mycomment}[3]{\ensuretext{\textcolor{#3}{[#1 #2]}}}
%disable comments here
\newcommand{\mycomment}[3]{}
\newcommand{\mc}[1]{\mycomment{\mcmarker}{#1}{magenta}}
\newcommand{\xn}[1]{\mycomment{\xnmarker}{#1}{blue}}
\newcommand{\mjm}[1]{\mycomment{\mjmarker}{#1}{cyan}}
\newcommand{\sa}[1]{\mycomment{\samarker}{#1}{orange}}
\newcommand{\ignore}[1]{}

